Greedy Gray Codes for some Restricted Classes of Binary Words

We investigate the existence of greedy Gray codes, based on the choice of the first element in the code, for two classes of binary words: generalized Fibonacci words and generalized Dyck words.

==> eptcsdata.tex <==
\providecommand{\firstpage}{108}
\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2024\\
EPTCS 403, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.403.23}{10.4204/EPTCS.403.23}}

